How to Design Sample and Computationally Efficient VQA Models

In multi-modal reasoning tasks, such as visual question answering (VQA), there have been many modeling and training paradigms tested. Previous models propose different methods for the vision and language tasks, but which ones perform the best while being sample and computationally efficient? Based on our experiments, we find that representing the text as probabilistic programs and images as object-level scene graphs best satisfy these desiderata. We extend existing models to leverage these soft programs and scene graphs to train on question answer pairs in an end-to-end manner. Empirical results demonstrate that this differentiable end-to-end program executor is able to maintain state-of-the-art accuracy while being sample and computationally efficient.

==> figures/intro_efficiency.tex <==
\begin{figure}[!t]
\centering
\resizebox{0.95\textwidth}{!}{%

\input{figures/plots/intro_text_efficiency}
\input{figures/plots/intro_vision_efficiency}
% \input{figures/plots/vision_efficiency_pretrain}
}
% \includegraphics[width=0.489\columnwidth]{figures/text_training.pdf}
% \includegraphics[width=0.489\columnwidth]{figures/vision_training.pdf}
\caption{Validation QA accuracy over the number of training samples at 10\% QA data. Each method was run 5 times. We record these accuracies over the number of samples used, which represents epochs $\times$ batch size for continuous methods or samples/replays for discrete.}
\label{fig:intro_stat_eff}
\end{figure}

==> figures/plot_efficiency.tex <==
% \usepgfplotslibrary{fillbetween}
\begin{figure}[!h]
\centering
\resizebox{0.95\textwidth}{!}{%

\input{figures/plots/text_efficiency}
\input{figures/plots/vision_efficiency_scratch}
\input{figures/plots/vision_efficiency_pretrain}
}
% \includegraphics[width=0.489\columnwidth]{figures/text_training.pdf}
% \includegraphics[width=0.489\columnwidth]{figures/vision_training.pdf}
\caption{Validation QA accuracy over the number of training samples at 10\% QA data. Each method was run 5 times. We record these accuracies over the number of samples used, which represents epochs $\times$ batch size for continuous methods or samples/replays for discrete.\bh{Try to be consistent among the subfigures, including the coloring scheme, and the shading.}}
\label{plt:effy}
\end{figure}

==> tables/e2e_all.tex <==
\begin{table}[!h]
    % \caption{Global caption}
    % \begin{minipage}{.51\linewidth}
    %     \resizebox{1.0\textwidth}{!}{%
    %     \begin{tikzpicture}
    %     \begin{axis}[
    %             ybar,
    %             symbolic x coords={0\%,1\%,5\%, 10\%, 100\%},
    %             xtick=data,
    %             % nodes near coords,
    %             xlabel = \% of QA Data,
    %             ylabel = Validation Accuracy,
    %             legend style={at={(0.5,-0.2)},anchor=north, legend columns=-1},
    %         ]
    %         % 01_pre  05_pre  1_pre
    %         \addplot table[x=perc_symb,y expr=\thisrow{01_pre}]{data/e2e_results.dat};
    %         \addplot table[x=perc_symb,y expr=\thisrow{05_pre}]{data/e2e_results.dat};
    %         \addplot table[x=perc_symb,y expr=\thisrow{1_pre}]{data/e2e_results.dat};
    %         \legend{0.1\% pre-train, 0.5\% pre-train, 1\% pre-train}
    %     \end{axis}
    %     \end{tikzpicture}
    %     }
    % \end{minipage}%
    % \begin{minipage}{.49\linewidth}
        \renewcommand{\arraystretch}{1.28}
        \centering
        \begin{tabular}{c c c}
        \toprule
        Method & 100\% Data & 10\% Data\\
        \midrule
        TbD & 99.1 & 54.2 \\
        MAC & 98.9 & 67.3 \\
        NS-CL & 99.2 & 98.8 \\
        NS-VQA & 99.8 & 92.1 \\
        LXMERT & 97.9 & 66.5 \\
        LC-GCN & 97.9 & 64.8 \\
        Stack-NMN & 96.3 & 86.8 \\
        NGS & \textbf{100.0} & 87.3* \\
        % NGS-RL & 96.9 & 80.0 \\
        \hline
        \PROJNAME \ (0.1\%) & 99.0 & 98.0 \\
        \PROJNAME \ (1.0\%) & 99.5 & \textbf{99.3} \\
        \bottomrule
        \end{tabular}
    % \end{minipage}
    \caption{Performance of our method on different training data percentages and pre-training. We also compare against other representative methods with our models with 0.1\% and 1\% pre-training. The 10\% result for NGS* was taken from the closest reported result at 25\% data. \bh{Add reference here after the baseline names if you have space}}
    \label{tab:e2e_all}
\end{table}


==> tables/e2e_perf.tex <==
% \begin{table}[h]
%     \centering
%     \begin{tabular}{cccc}
%         %  \cline{2-4}
%         %  \multicolumn{1}{c}{} & \multicolumn{3}{|c|}{\% pre-training data} \\
%         \cline{2-4}
%         \multicolumn{1}{c}{} & \multicolumn{3}{c}{\% pre-training data} \\
%         \hline
%         \% QA labels & 0.1 & 0.5 & 1 \\ 
%         \hline
%         0 & 47.0 & 73.1 & 95.5 \\
%         1 & 65.4& & 98.0 \\  
%         5 & & & 98.7 \\
%         10 & & & 99.1\\
%         100  & & & 99.4\\
%         \hline
%     \end{tabular}
%     \caption{Validation accuracy given different amount of fine pre-training data and coarse question answer labels.}
%     \label{tab:val_qa_acc}
% \end{table}

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.9\textwidth]{figures/joint_results_v1.png}
\end{center}
\caption{Validation accuracy of our approach on CLEVR dataset given different amount of fine pre-training data and question answer labels.}
\end{figure}

==> tables/intro_samp_perf.tex <==
\begin{table*}[!t]
    % \caption{Global caption}
    \begin{minipage}{.45\linewidth}
        \centering
        \begin{tabular}{c| c c}
        \toprule
        QA & Symbolic Progs. & Soft Progs. \\
        Data \% & NS-VQA & Stack-NMN\\
        \midrule
        1\% & \textbf{86.5} &  \\
        5\% & 89.2 &  \\
        10\% & 92.1 &  \\
        \bottomrule
        \end{tabular}
        \caption{QA accuracy when testing sample efficiency of language components with frozen fine tuned vision.}
        \label{tab.text_sample}
    \end{minipage}%
    \hfill
    \begin{minipage}{.5\linewidth}
        \centering
        \begin{tabular}{c| c c c}
        \toprule
        & Pixel-wise & Object-level & Object-level \\
        QA & NMN & Symb. Logic & Soft Logic \\
        Data \% & Stack-NMN & NS-VQA & NS-CL \\
        \midrule
        1\% & 47.1 & 92.6 & \textbf{96.1} \\
        5\% & 66.8 & 96.2 & \textbf{97.2} \\
        10\% & 93.5 & 97.2 & \textbf{98.8} \\
        \bottomrule
        \end{tabular}
        \caption{QA accuracy when testing sample efficiency of vision components with frozen fine tuned program parsers.}
        \label{tab.vision_sample}
    \end{minipage} 
\end{table*}



==> tables/loss_weights.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{c c c c}
        \toprule
        \% QA Data & 0.1\% & 0.5\% & 0.1\% \\
        \midrule
        5\% & & & \\
        10\% & & & \\
        100\% & & & \\
        \bottomrule
    \end{tabular}
    \caption{Performance gains by adding pre-training loss weights.}
    \label{tab:loss_weights}
\end{table}

==> text/prev_notes.tex <==
\subsection{Definitions for operators, programs and memory}

For each sample we are given an image I and a natural language question Q. We also have prior knowledge about a domain specific language (DSL) that could solve Q through executing the correct functional program over I's scene graph G. There are individual functions that compose this DSL such as $\{\texttt{filter, relate, exist, sum}\} \in \mathcal{F}$.

The image I can be processed into its feature and locations $I_{feat}, I_{loc}$ through an object detection step with a trained classifier. Unsupervised or low shot detections would be the most ideal, as we are working in the low data scenario, thus would bottleneck the pipeline (see AB-VQA reviews). This would be an interesting CV direction to explore. Similarly the question Q can be mapped into an embedding matrix of the individual words $T_{feat}$.

We have global inputs available at each step of execution, which are $I_{feat}, I_{loc}, T_{feat}$ and the memory $M$. The memory is responsible for storing the intermediate steps of the execution. This is necessary as each function may require different numbers of previous inputs, so a global state of the results are kept in a stack.

\subsection{Overall Model}

\Le{Please include a picture a picture for the overall model.} 

To generate the answer from I and Q, we require to sequentially execute the correct functions over the detected objects to find the answer. These intermediate executions are handled by visual question reasoning (VQR) cells, which handle the uncertainty in choosing a specific function at each step through a weighted average. A fixed number $T$ of these VQR cells are assembled and executed sequentially. The output from the final cell execution can be used to answer the question. The execution of the cells can be seen in Algorithm~ \ref{alg:overview}.

\begin{algorithm}[H]
\SetAlgoLined
\KwResult{final $M_T$}
 $I_{feat}, I_{loc}$ = FRCNN(I)\;
 $q = $ Embed(Q) \;
 $S = |Q|$ \;
 $h = [h_1, \hdots, h_{|Q|}] =  \text{Bi-LSTM}(q; \theta_{lstm})$ \;
 $q_{ave} = \frac{\sum_{s=1}^S q_s}{S}$\;
 $M = $ empty\_stack \;
 $c_0 = \vec{0}$ \;
 \For{i in [1, T]}{
    $w_i, c_i = \text{text\_encoder}(h, i, c_{i-1}, q_{ave})$ \tcp{attention distribution over the functions}
    M.push($\text{VQR}(w_i, c_i)$) \tcp{compute expected output and update memory}
 }
 return M.pop()
\caption{Model(I, Q) question answering iteration}
\label{alg:overview}
\end{algorithm}

\subsubsection{Language and Vision Encoders}
The text\_encoder uses a recurrent model to perform attention computations each unrolled step $i$. Following \citet{stack_nmn}, we leverage a Bi-LSTM method to encode the function probability distribution $w_i$. Additionally the most relevant question word embeddings are encoded within a context vector $c_i$. The $w_i$ and $c_i$ are passed to the VQR cell which uses the former to weight all functions $\mathcal{F}$ outputs and the latter within each function to determine which attribute it is trying to predict. This is outlined in Algorithm \ref{alg:encoder}.

% This Such methods could be a coarse-to-fine decoder (\cite{dong2018coarse}) where $\mathcal{F}$ is the coarse sketch of the functions needed and their corresponding probabilities $F_a$. The sketches are correspondingly used to fill in the function parameters such as $\texttt{filter}(F_{in}; I_{feat}; I_{loc}; \texttt{[red, small]})$. These functions have corresponding image classifiers that can select the detected objects from the image given the function parameters

% If the attention corresponding to the termination function $\mathcal{F}_{END}$ indicating the end of the execution. It will return the previous memory location . This retrieved memory row $M_i$ can be used to retrieve the corresponding answer based on its position. This position is determined by taking the most probable component based on $w_{i-1}$ to extract the relevant region for supervision.

\begin{algorithm}[H]
\SetAlgoLined
\KwResult{$w_i$ and $c_i$}
 $u = W_2[W_1^i q_{ave} + b_1; c_{i-1}] + b_2$ \tcp{use prev distribution to guide next}
 $w_i = $ softmax(MLP(u; $\theta_{weight}$)) \;
 \For{s in [1, S]}{
    $cv_{i,s} = \text{sigmoid}(W_3(u \odot h_s))$ \tcp{scalar word attention}
 }
 $c_i = \sum_{s=1}^S cv_{i,s} \cdot h_s$ \;
 return $w_i, c_i$
\caption{$\text{text\_encoder}(h, i, c_{i-1}, q_{ave})$ execution}
\label{alg:encoder}
\end{algorithm}

In addition to the weights and context, we have to predict the probability distribution of arguments $p_{arg}$ per function. This is done through another small MLPs. If we are in the \texttt{filter\_color} function and want to predict the distribution of colors: $p_{arg} = \text{MLP}(c_i; \theta_{arg}^{color})$.

The vision models are MLPs as well. These vision models predict the visual attributes of the objects detected by the Faster RCNN. Similarly in the \texttt{filter\_color}, given the image feature of an object $i$ we predict the color attribute as $p_{attr}^i = \text{MLP}(I_{feat}^i; \theta_{attr}^{color})$. We are also interested in modeling the relations between objects which can be calculated per object. To calculate the relation for object $i$ with respect to all other objects we perform $p_{rel}^i = \text{MLP}(I_{loc}^i, I_{loc}; \theta_{rel})$.

We highlight that $\theta^{arg}$ and $\theta^{attr}$ are encoding different modalities. The former is estimating what the function arguments are based on the context text embedding while the latter is predicting the attributes of the visual objects themselves. This information will be joined appropriately by the modular functions.

The full set of trainable text models are $\Theta_T = \{\theta_{lstm}, \theta_{weight}, \theta_{arg}^*\}$, $\Theta_V = \{\theta_{attr}^*, \theta_{rel}\}$ and for the vision.


% \subsubsection{VQR Cells}
% In the VQR cell we execute each function in $\mathcal{F}$ and weight their outputs using $w_i$. A special function $\mathcal{F}_{END}$ indicates the end of the execution. Any subsequent $\mathcal{F}_{END}$ predicted functions will just copy the previous memory until time $T$ to preserve the final answer. The final $M_T$ is used for final supervision.

